HG-PIPE: Vision Transformer Acceleration with Hybrid-Grained Pipeline

Vision Transformer (ViT) acceleration with field programmable gate array (FPGA) is promising but challenging. Existing FPGA-based ViT accelerators mainly rely on temporal architectures, which process different operators by reusing the same hardware blocks and suffer from extensive memory access overhead. Pipelined architectures, either coarse-grained or fine-grained, unroll the ViT computation spatially for memory access efficiency. However, they usually suffer from significant hardware resource constraints and pipeline bubbles induced by the global computation dependency of ViT. In this paper, we introduce HG-PIPE, a pipelined FPGA accelerator for high-throughput and low-latency ViT processing. HG-PIPE features a hybrid-grained pipeline architecture to reduce on-chip buffer cost and couples the computation dataflow and parallelism design to eliminate the pipeline bubbles. HG-PIPE further introduces careful approximations to implement both linear and non-linear operators with abundant Lookup Tables (LUTs), thus alleviating resource constraints. On a ZCU102 FPGA, HG-PIPE achieves 2.78 times better throughput and 2.52 times better resource efficiency than the prior-art accelerators, e.g., AutoViTAcc. With a VCK190 FPGA, HG-PIPE realizes end-to-end ViT acceleration on a single device and achieves 7118 images/s, which is 2.81 times faster than a V100 GPU.

==> docs/8-citation.tex <==
%-------------------------------------------------------------------------------



==> docs/rebuttal.tex <==
Thank you for your insightful comments on our work. We acknowledge the concerns raised and have addressed them as follows:

Q1: The generality of HG-PIPE — this paper only optimizes a specific size of ViT (Deit-tiny), and there are many hand-crafted designs just for fitting this model onto two FPGA platforms. How does it adapt to different sizes? For example, for a larger ViT model, will we still have enough LUTs? Will we still get such performance improvements? (The paper only discusses a specific size of ViT and specific hardware platforms. It is unclear how general the design is.)

A1: Our design is template-based and therefore highly scalable, and we can adjust the template parameters to adapt to ViT-small and ViT-base models. Here we provide some representative template parameters of the attention layer. H: attention head numbers; TP: token parallelism; MATMUL_QKV_CIP and MATMUL_QKV_COP: input and output channel parallelism in QKV generation; attn_if_t: input feature map data type; attn_lnq_t: layernorm quantization result data type. The template allows flexible adjustments of such hyperparameters, therefore enabling the scalability of our design.

Regarding your concern about the sufficiency of LUTs for larger models, it's important to note that we can accommodate larger models by properly scaling down the parallelism of each layer. For instance, reducing the parallelism to 1/14 would allow us to accelerate the ViT-base at 510 frames per second with the same LUT cost. Furthermore, our asynchronized pipelined network structure can be easily extended across multiple FPGA platforms. Boards can be interconnected using high-speed SerDes, enhancing both the scalability of the model and the flexibility of the hardware platform. Since the resource efficiency will be consistent, on larger models, our work will keep the performance advantage beyond other works.

Q2: Is it possible to design an automatic compilation/HLS tool that can adapt to different model sizes? Can the whole of Section 4.3 be automatic? (Not enough explanation of the process used to calculate parallelism designs, like any formulae, empirical data, or optimization algorithms. It is fully hand-tuned or can it be automatic?)

A2: Automatic accelerator generation with design space exploration (DSE) is a fascinating topic. In CNNs, each layer has a different size, leading to a vast and exponentially growing design space. Therefore, many CNN accelerator works tried DSE to achieve higher resource efficiency with a given throughput requirement. However, this is not the case for ViTs. Transformer architectures maintain the same layer size throughout, leading to a very small design space. This smaller design space makes manual design feasible and can often yield optimal results without the need for automation. Even for several different model sizes, hand designing is capable enough. Also, integrating design automation into our design would blur the focus of our work: solving the granularity problem in attention. As for the parallelism designs, we have provided several necessary formulas in Section 4.3 to explain the BRAM efficiency and the divisibility-driven design constraints. We recognized that we might have ignored some formulas, and we provided them here. The parallelism calculation formula, P = TP x CIP x COP, which means the total parallelism is the product of the parallelism along all dimensions. The Initiation Interval (II) will be II= Cycles / P, which means the design will produce 1 tensor every II cycles. Cycles = T x CI x CO, which is the complexity of the matrix multiplication. FPS = frequency / II, e.g., 425MHz / 57624 = 7375 frames per second. We achieved 7248 FPS, which is close to the ideal result.

Q3: In Table 6, the comparison is not apple-to-apple. Only HeatViT runs the same Deit-tiny as HG-PIPE, and HeatViT uses a very different quantization (A8W8 vs HG-PIPE’s A4W4 and A3W3). I am not sure how to read this table. (The experiments' setup differs from various baselines. The results may not be comparable.)  

A3: In the area of FPGA-based accelerators, the apple-to-apple comparison is very difficult, and we have tried our best to collect SOTA and comparable works. ViT-tiny shares the same structure as Deit-tiny, therefore we have two competitors with the same architecture. As for the quantization, we can achieve better accuracy in a lower precision  (e.g. 74.37%@A4W4  in our work and 72.20%@A8W8 in HeatViT), which should be considered an advantage of our work. Almost all accelerator works suffer from this comparison problem, and some works even choose not to compare with related works (e.g. HeatViT, AutoViTAcc, VAQF) and only compare with their own baseline implementations. We have tried our best to do a fair comparison, traversing more than 30 papers and choosing the most representative works. I hope our explanation can address your concern.

Q4: Figure 17: the model accuracy is still slightly impacted by 0.3%. In some places, the paper claims “without compromising model accuracy”, e.g., in Conclusion on the same page. Is it over-claim? Will the gap enlarge for larger models?

A4: Indeed, our non-linear function approximation caused a 0.3% accuracy drop. However, a 0.3% degradation is really a very small accuracy drop in hardware accelerator designs. Most accelerators will suffer more than 1% accuracy degradation. For example, SSR will suffer a 1% degradation for its most accurate setup, and HeatViT has a 2% degradation. Some works will suffer even higher degradation up to 5%, e.g. FixyFPGA. Some works even don’t provide their accuracy, e.g. ViA. From a hardware designer's perspective, considering we greatly reduced the DSP cost, the 0.3% degradation is negligible. Currently we don’t know whether the gap will enlarge for larger models, but we believe that we can increase the size of the lookup table to compensate for the impact.

Finally, thank you for your efforts in reviewing our work, and also for your insightful comments!
